Transformer Vs. MLP-Mixer: Exponential Expressive Gap For NLP Problems

Vision-Transformers are widely used in various vision tasks. Meanwhile, there is another line of works starting with the MLP-mixer trying to achieve similar performance using mlp-based architectures. Interestingly, until now those mlp-based architectures have not been adapted for NLP tasks. Additionally, until now, mlp-based architectures have failed to achieve state-of-the-art performance in vision tasks. In this paper, we analyze the expressive power of mlp-based architectures in modeling dependencies between multiple different inputs simultaneously, and show an exponential gap between the attention and the mlp-based mechanisms. Our results suggest a theoretical explanation for the mlp inability to compete with attention-based mechanisms in NLP problems, they also suggest that the performance gap in vision tasks may be due to the mlp relative weakness in modeling dependencies between multiple different locations, and that combining smart input permutations with mlp architectures may not be enough to close the performance gap alone.

==> cvpr2023-author_kit-v1_1-1/all/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> cvpr2023-author_kit-v1_1-1/all/tab-desth.tex <==
\begin{table}
\resizebox{\columnwidth}{!}{
\setlength{\tabcolsep}{0.36em}
\begin{tabular}{c|cc|cc|cc|cc|cc}
	\toprule

	\multirow{2}{*}{\backslashbox{$H_\mathsf{S}$}{$H_\mathsf{D}$}} & \multicolumn{2}{c|}{Random} & \multicolumn{2}{c|}{Semihard} & \multicolumn{2}{c|}{Softhard} & \multicolumn{2}{c|}{Distance} & \multicolumn{2}{c}{Hardest}\tabularnewline
\cline{2-11} \cline{3-11} \cline{4-11} \cline{5-11} \cline{6-11} \cline{7-11} \cline{8-11} \cline{9-11} \cline{10-11} \cline{11-11} 
& R@1 & ERS & R@1 & ERS & R@1 & ERS & R@1 & ERS & R@1 & ERS\tabularnewline

\midrule

Random & \cellcolor{black!7}53.9 & \cellcolor{black!7}3.8 & 27.0 & 35.1 & \multicolumn{2}{c|}{Collapse} & \multicolumn{2}{c|}{Collapse} & \multicolumn{2}{c}{Collapse}\tabularnewline
%\hline
Semihard & 43.9 & 5.4 & \cellcolor{black!7}44.0 & \cellcolor{black!7}5.0 & \multicolumn{2}{c|}{Collapse} & \multicolumn{2}{c|}{Collapse} & \multicolumn{2}{c}{Collapse}\tabularnewline
%\hline
Softhard & 48.3 & 13.7 & 38.4 & 29.6 & \cellcolor{black!7}55.7 & \cellcolor{black!7}6.2 & \multicolumn{2}{c|}{Collapse} & \multicolumn{2}{c}{Collapse}\tabularnewline
%\hline
Distance & 52.7 & 4.8 & 50.7 & 4.8 & \multicolumn{2}{c|}{Collapse} & \cellcolor{black!7}51.4 & \cellcolor{black!7}4.9 & 54.7 & 5.4\tabularnewline
%\hline
Hardest & 51.0 & 4.7 & 52.2 & 4.8 & \multicolumn{2}{c|}{Collapse} & 52.6 & 5.1 & \cellcolor{black!7}48.9 & \cellcolor{black!7}5.0\tabularnewline

	\bottomrule
\end{tabular}
}
%
	\vspace{-0.5em}
%
\caption{Combinations of source \& destination hardness.
	%
	Evaluated on the CUB Dataset with RN18 model.
	%
	The last-epoch performance is reported instead of the peak performance for alignment.
	%
	Models on the diagonal are regularly (instead of adversarially) trained.
	%
}
	\label{tab:desth}

\end{table}


==> cvpr2023-author_kit-v1_1-1/all/tab-gaeff.tex <==
\begin{table*}
\resizebox{\linewidth}{!}{
\setlength{\tabcolsep}{0.48em}
\renewcommand{\arraystretch}{1.02}%

\begin{tabular}{c|cc|cccc|ccccc|ccccc|c}

	\toprule

\rowcolor{black!12} & & & \multicolumn{4}{c|}{\textbf{Benign Example}} & \multicolumn{10}{c|}{\textbf{White-Box Attacks for Robustness Evaluation}} & \tabularnewline
\cline{4-17} \cline{5-17} \cline{6-17} \cline{7-17} \cline{8-17} \cline{9-17} \cline{10-17} \cline{11-17} \cline{12-17} \cline{13-17} \cline{14-17} \cline{15-17} \cline{16-17} \cline{17-17}
\rowcolor{black!12}\multirow{-2}{*}{\textbf{Dataset}} &  \multirow{-2}{*}{\textbf{Defense}} & \multirow{-2}{*}{$\eta$}  & R@1$\uparrow$ & R@2$\uparrow$ & mAP$\uparrow$ & NMI$\uparrow$ & CA+$\uparrow$ & CA-$\downarrow$ & QA+$\uparrow$ & QA-$\downarrow$ & TMA$\downarrow$ & ES:D$\downarrow$ & ES:R$\uparrow$ & LTM$\uparrow$ & GTM$\uparrow$ & GTT$\uparrow$ & \multirow{-2}{*}{\textbf{ERS$\uparrow$}}\tabularnewline

	\midrule

& \textcolor{tab:red}{HM{[}$\mathcal{S},\mathcal{M}${]}} & 8 & 38.4 & 49.7 & 22.9 & 50.3 & 10.9 & 50.5 & 10.8 & 44.6 & 0.680 & 0.722 & 13.3 & 11.2 & 25.8 & 1.2 & 29.6\tabularnewline
	\cline{2-18}
 & HM{[}$\mathcal{S},g_{\mathsf{B}}(\mathcal{M})${]} ($\xi=0.1$) & 8 & 36.5 & 48.0 & 21.4 & 48.4 & 13.0 & 44.0 & 13.2 & 35.6 & 0.667 & 0.628 & 20.3 & 13.2 & 26.7 & 2.8 & 33.8\tabularnewline
\rowcolor{black!7}\cellcolor{white} & HM{[}$\mathcal{S},0${]} & 8 & 0.8 & 0.9 & 0.8 & 6.0 & 19.8 & 92.4 & 42.0 & 51.9 & 1.000 & 0.000 & 1.2 & 1.2 & 1.0 & 14.1 & 29.7\tabularnewline
 & HM{[}$\mathcal{S},-\gamma/2${]} & 8 & 36.8 & 47.9 & 21.7 & 48.5 & 12.7 & 41.5 & 12.2 & 35.7 & 0.668 & 0.633 & 18.1 & 14.3 & 28.4 & 2.9 & 33.8\tabularnewline
\rowcolor{black!7}\cellcolor{white} & HM{[}$\mathcal{S},-\gamma${]} & 8 & 37.8 & 48.1 & 22.1 & 48.7 & 11.7 & 48.4 & 11.3 & 43.2 & 0.541 & 0.850 & 15.2 & 11.6 & 26.1 & 1.3 & 31.2\tabularnewline
\multirow{-6}{*}{CUB}  & \textcolor{tab:pink}{HM{[}$\mathcal{S},g_{\mathsf{LGA}}${]}} & 8 & 38.0 & 48.3 & 21.8 & 49.3 & 12.7 & 46.4 & 11.6 & 39.9 & 0.567 & 0.783 & 16.8 & 11.9 & 27.9 & 1.4 & 32.4\tabularnewline

	\hline

\multirow{5}{*}{CUB} & HM{[}$\mathcal{S},-\gamma/2${]} & 2 & 44.5 & 55.9 & 27.6 & 53.3 & 2.4 & 86.1 & 1.3 & 87.7 & 0.809 & 1.091 & 1.5 & 1.8 & 22.1 & 0.1 & 12.4\tabularnewline
\rowcolor{black!7}\cellcolor{white} & HM{[}$\mathcal{S},-\gamma/2${]} & 4 & 40.0 & 50.7 & 23.8 & 50.3 & 8.0 & 59.8 & 7.5 & 55.5 & 0.694 & 0.860 & 10.2 & 6.5 & 26.2 & 0.4 & 24.7\tabularnewline
 & HM{[}$\mathcal{S},-\gamma/2${]} & 8 & 36.8 & 47.9 & 21.7 & 48.5 & 12.7 & 41.5 & 12.2 & 35.7 & 0.668 & 0.633 & 18.1 & 14.3 & 28.4 & 2.9 & 33.8\tabularnewline
\rowcolor{black!7}\cellcolor{white} & HM{[}$\mathcal{S},-\gamma/2${]} & 16 & 35.2 & 45.8 & 20.3 & 47.6 & 15.0 & 36.3 & 15.1 & 30.7 & 0.638 & 0.595 & 19.6 & 16.8 & 28.7 & 3.5 & 36.8\tabularnewline
 & HM{[}$\mathcal{S},-\gamma/2${]} & 32 & 34.7 & 45.5 & 20.0 & 47.5 & 15.0 & 36.7 & 15.1 & 29.9 & 0.631 & 0.611 & 20.1 & 17.2 & 29.3 & 3.5 & 37.0\tabularnewline
\hline
\multirow{5}{*}{CUB} & \textcolor{tab:pink}{HM{[}$\mathcal{S},g_{\mathsf{LGA}}${]}} & 2 & 47.5 & 59.3 & 30.1 & 55.3 & 1.8 & 88.1 & 1.1 & 88.9 & 0.854 & 1.022 & 2.3 & 0.8 & 21.2 & 0.0 & 11.7\tabularnewline
\rowcolor{black!7}\cellcolor{white} & \textcolor{tab:pink}{HM{[}$\mathcal{S},g_{\mathsf{LGA}}${]}} & 4 & 42.7 & 53.6 & 26.3 & 52.6 & 6.5 & 67.3 & 4.6 & 65.0 & 0.734 & 0.893 & 6.6 & 5.8 & 23.7 & 0.3 & 20.8\tabularnewline
 & \textcolor{tab:pink}{HM{[}$\mathcal{S},g_{\mathsf{LGA}}${]}} & 8 & 38.0 & 48.3 & 21.8 & 49.3 & 12.7 & 46.4 & 11.6 & 39.9 & 0.567 & 0.783 & 16.8 & 11.9 & 27.9 & 1.4 & 32.4\tabularnewline
\rowcolor{black!7}\cellcolor{white} & \textcolor{tab:pink}{HM{[}$\mathcal{S},g_{\mathsf{LGA}}${]}} & 16 & 37.0 & 47.2 & 21.3 & 48.4 & 13.6 & 42.2 & 13.1 & 35.9 & 0.533 & 0.757 & 16.3 & 15.3 & 27.2 & 2.1 & 34.5\tabularnewline
 & \textcolor{tab:pink}{HM{[}$\mathcal{S},g_{\mathsf{LGA}}${]}} & 32 & 36.5 & 46.7 & 21.0 & 48.6 & 14.7 & 39.6 & 15.6 & 34.2 & 0.523 & 0.736 & 16.5 & 15.0 & 26.7 & 2.9 & 35.9\tabularnewline
 
	\bottomrule

\end{tabular}

	}
	\vspace{-0.8em}
\caption{Effectiveness of gradual adversary as $H_\mathsf{D}$ in hardness manipulation.}
\label{tab:gaeff}
\end{table*}


==> cvpr2023-author_kit-v1_1-1/all/tab-hmeff.tex <==
\begin{table*}
\resizebox{\linewidth}{!}{
\setlength{\tabcolsep}{0.48em}%
\renewcommand{\arraystretch}{1.05}

\begin{tabular}{c|cc|cccc|ccccc|ccccc|c}

	\toprule

\rowcolor{black!12} & & & \multicolumn{4}{c|}{\textbf{Benign Example}} & \multicolumn{10}{c|}{\textbf{White-Box Attacks for Robustness Evaluation}} & \tabularnewline
\cline{4-17} \cline{5-17} \cline{6-17} \cline{7-17} \cline{8-17} \cline{9-17} \cline{10-17} \cline{11-17} \cline{12-17} \cline{13-17} \cline{14-17} \cline{15-17} \cline{16-17} \cline{17-17}
\rowcolor{black!12}\multirow{-2}{*}{\textbf{Dataset}} & \multirow{-2}{*}{\textbf{Defense}} & \multirow{-2}{*}{$\eta$} & R@1$\uparrow$ & R@2$\uparrow$ & mAP$\uparrow$ & NMI$\uparrow$ & CA+$\uparrow$ & CA-$\downarrow$ & QA+$\uparrow$ & QA-$\downarrow$ & TMA$\downarrow$ & ES:D$\downarrow$ & ES:R$\uparrow$ & LTM$\uparrow$ & GTM$\uparrow$ & GTT$\uparrow$ & \multirow{-2}{*}{\textbf{ERS$\uparrow$}}\tabularnewline

	\midrule

CUB & N/A{[}$\mathcal{R}${]} & N/A & 53.9 & 66.4 & 26.1 & 59.5 & 0.0 & 100.0 & 0.0 & 99.9 & 0.883 & 1.762 & 0.0 & 0.0 & 14.1 & 0.0 & 3.8\tabularnewline
\hline
\multirow{5}{*}{CUB} & \textcolor{tab:cyan}{ACT{[}$\mathcal{R}${]}}\cite{robrank} & 2 & 46.5 & 58.4 & 29.1 & 55.6 & 0.6 & 98.9 & 0.4 & 98.1 & 0.837 & 1.666 & 0.2 & 0.2 & 19.6 & 0.0 & 5.8\tabularnewline
\rowcolor{black!7}\cellcolor{white} & \textcolor{tab:cyan}{ACT{[}$\mathcal{R}${]}}\cite{robrank} & 4 & 38.4 & 49.8 & 22.8 & 49.7 & 4.6 & 81.9 & 2.8 & 80.5 & 0.695 & 1.366 & 2.9 & 2.3 & 18.8 & 0.1 & 13.9\tabularnewline
 & \textcolor{tab:cyan}{ACT{[}$\mathcal{R}${]}}\cite{robrank} & 8 & 30.6 & 40.1 & 16.5 & 45.6 & 13.7 & 46.8 & 12.6 & 39.3 & 0.547 & 0.902 & 13.6 & 9.8 & 21.9 & 1.3 & 31.3\tabularnewline
\rowcolor{black!7}\cellcolor{white} & \textcolor{tab:cyan}{ACT{[}$\mathcal{R}${]}}\cite{robrank} & 16 & 28.6 & 38.7 & 15.1 & 43.7 & 15.8 & 37.9 & 16.0 & 31.5 & 0.496 & 0.834 & 11.3 & 9.8 & 21.2 & 2.1 & 34.7\tabularnewline
 & \textcolor{tab:cyan}{ACT{[}$\mathcal{R}${]}}\cite{robrank} & 32 & 27.5 & 38.2 & 12.2 & 43.0 & 15.5 & 37.7 & 15.1 & 32.2 & 0.472 & 0.821 & 11.1 & 9.4 & 14.9 & 1.0 & 33.9\tabularnewline
\hline
\multirow{5}{*}{CUB} & \textcolor{tab:orange}{ACT{[}$\mathcal{S}${]}}\cite{robrank} & 2 & 53.0 & 65.1 & 34.7 & 59.9 & 0.0 & 100.0 & 0.0 & 99.8 & 0.877 & 1.637 & 0.0 & 0.0 & 20.4 & 0.0 & 5.1\tabularnewline
\rowcolor{black!7}\cellcolor{white}& \textcolor{tab:orange}{ACT{[}$\mathcal{S}${]}}\cite{robrank} & 4 & 49.3 & 61.0 & 31.5 & 56.6 & 0.6 & 97.6 & 0.2 & 98.1 & 0.799 & 1.485 & 0.3 & 0.2 & 18.9 & 0.0 & 7.1\tabularnewline
& \textcolor{tab:orange}{ACT{[}$\mathcal{S}${]}}\cite{robrank} & 8 & 42.8 & 54.7 & 26.6 & 53.3 & 4.8 & 72.8 & 2.7 & 73.3 & 0.619 & 1.148 & 8.3 & 4.9 & 23.5 & 0.3 & 18.7\tabularnewline
\rowcolor{black!7}\cellcolor{white}& \textcolor{tab:orange}{ACT{[}$\mathcal{S}${]}}\cite{robrank} & 16 & 40.5 & 51.6 & 24.8 & 51.7 & 6.7 & 62.1 & 4.9 & 60.6 & 0.566 & 1.014 & 12.4 & 8.6 & 22.5 & 0.9 & 23.7\tabularnewline
& \textcolor{tab:orange}{ACT{[}$\mathcal{S}${]}}\cite{robrank} & 32 & 39.4 & 50.2 & 18.6 & 51.3 & 6.8 & 61.5 & 5.2 & 60.4 & 0.506 & 1.032 & 12.8 & 11.3 & 17.7 & 0.3 & 24.2\tabularnewline
\hline
\multirow{5}{*}{CUB} & \textcolor{tab:blue}{HM{[}$\mathcal{R},\mathcal{M}${]}} & 2 & 34.3 & 44.9 & 19.5 & 47.4 & 7.7 & 77.5 & 6.5 & 70.8 & 0.636 & 1.281 & 4.3 & 2.6 & 21.1 & 0.2 & 18.1\tabularnewline
\rowcolor{black!7}\cellcolor{white} & \textcolor{tab:blue}{HM{[}$\mathcal{R},\mathcal{M}${]}} & 4 & 30.7 & 40.3 & 16.4 & 45.3 & 13.9 & 60.4 & 13.5 & 48.1 & 0.582 & 1.041 & 6.6 & 6.6 & 20.2 & 1.2 & 27.1\tabularnewline
 & \textcolor{tab:blue}{HM{[}$\mathcal{R},\mathcal{M}${]}} & 8 & 27.0 & 36.0 & 13.2 & 42.5 & 19.4 & 48.0 & 22.2 & 32.0 & 0.535 & 0.867 & 11.6 & 10.4 & 19.3 & 2.9 & 35.1\tabularnewline
\rowcolor{black!7}\cellcolor{white} & \textcolor{tab:blue}{HM{[}$\mathcal{R},\mathcal{M}${]}} & 16 & 23.8 & 32.6 & 11.6 & 40.6 & 20.9 & 45.0 & 24.6 & 28.6 & 0.494 & 0.805 & 15.6 & 11.3 & 22.1 & 3.2 & 38.0\tabularnewline
 & \textcolor{tab:blue}{HM{[}$\mathcal{R},\mathcal{M}${]}} & 32 & 23.1 & 31.9 & 11.3 & 40.3 & 22.8 & 46.0 & 24.3 & 28.3 & 0.495 & 0.800 & 14.2 & 11.7 & 19.7 & 3.8 & 38.0\tabularnewline
\hline
\multirow{5}{*}{CUB} & \textcolor{tab:red}{HM{[}$\mathcal{S},\mathcal{M}${]}} & 2 & 44.5 & 56.1 & 27.8 & 53.3 & 1.9 & 87.7 & 1.6 & 88.8 & 0.827 & 1.101 & 3.7 & 0.3 & 19.0 & 0.0 & 11.6\tabularnewline
\rowcolor{black!7}\cellcolor{white} & \textcolor{tab:red}{HM{[}$\mathcal{S},\mathcal{M}${]}} & 4 & 40.6 & 51.8 & 24.2 & 51.0 & 7.3 & 64.1 & 6.3 & 60.9 & 0.715 & 0.894 & 7.9 & 4.4 & 22.8 & 0.2 & 22.1\tabularnewline
 & \textcolor{tab:red}{HM{[}$\mathcal{S},\mathcal{M}${]}} & 8 & 38.4 & 49.7 & 22.9 & 50.3 & 10.9 & 50.5 & 10.8 & 44.6 & 0.680 & 0.722 & 13.3 & 11.2 & 25.8 & 1.2 & 29.6\tabularnewline
\rowcolor{black!7}\cellcolor{white} & \textcolor{tab:red}{HM{[}$\mathcal{S},\mathcal{M}${]}} & 16 & 37.4 & 47.3 & 21.0 & 48.2 & 14.4 & 42.0 & 14.8 & 34.7 & 0.599 & 0.693 & 17.5 & 14.4 & 26.5 & 2.4 & 34.8\tabularnewline
 & \textcolor{tab:red}{HM{[}$\mathcal{S},\mathcal{M}${]}} & 32 & 35.3 & 46.1 & 20.2 & 48.0 & 15.1 & 41.8 & 15.2 & 33.0 & 0.589 & 0.686 & 18.7 & 14.9 & 27.8 & 2.9 & 35.7\tabularnewline

	\bottomrule

\end{tabular}

} \vspace{-0.5em}
	%
\caption{Hardness manipulation in adversarial training.
%
The ``$\uparrow$'' mark means ``the higher the better'', while ``$\downarrow$''
	means the opposite.
%
	}
	%
\label{tab:hmeff}
%
\end{table*}


==> cvpr2023-author_kit-v1_1-1/all/tab-hsort.tex <==
\begin{table}
\resizebox{\columnwidth}{!}{
	\setlength{\tabcolsep}{0.8em}
\begin{tabular}{c|ccccc}
\toprule
\rowcolor{black!7} Statistics & Random & Semihard & Softhard & Distance & Hardest\tabularnewline
\midrule
$E[H]$ & $-0.164$ & $-0.126$ & $-0.085$ & $0.043$ & $0.044$\tabularnewline
$\text{Var}[H]$ & $0.00035$ & $0.00013$ & $0.00122$ & $0.00021$ & $0.00021$\tabularnewline
\bottomrule
\end{tabular}
}
	\vspace{-0.5em}
\caption{Mean \& variance of hardness w/ various triplet samplers.
%
Calculated as the average statistics over $1000$ mini-batches from the CUB dataset
with an imagenet-initialized RN18 model.
%
}

	\label{tab:hsort}
\end{table}


==> cvpr2023-author_kit-v1_1-1/all/tab-ics.tex <==
\begin{table*}
	\vspace{-1em}
\resizebox{\linewidth}{!}{
\setlength{\tabcolsep}{0.48em}
\renewcommand{\arraystretch}{1.02}%

\begin{tabular}{c|cc|cccc|ccccc|ccccc|c}

	\toprule

\rowcolor{black!12} & &  & \multicolumn{4}{c|}{\textbf{Benign Example}} & \multicolumn{10}{c|}{\textbf{White-Box Attacks for Robustness Evaluation}} & \tabularnewline
\cline{4-17} \cline{5-17} \cline{6-17} \cline{7-17} \cline{8-17} \cline{9-17} \cline{10-17} \cline{11-17} \cline{12-17} \cline{13-17} \cline{14-17} \cline{15-17} \cline{16-17} \cline{17-17}
\rowcolor{black!12}\multirow{-2}{*}{\textbf{Dataset}} & \multirow{-2}{*}{\textbf{Defense}} & \multirow{-2}{*}{$\eta$} & R@1$\uparrow$ & R@2$\uparrow$ & mAP$\uparrow$ & NMI$\uparrow$ & CA+$\uparrow$ & CA-$\downarrow$ & QA+$\uparrow$ & QA-$\downarrow$ & TMA$\downarrow$ & ES:D$\downarrow$ & ES:R$\uparrow$ & LTM$\uparrow$ & GTM$\uparrow$ & GTT$\uparrow$ & \multirow{-2}{*}{\textbf{ERS$\uparrow$}}\tabularnewline

	\midrule

& \textcolor{tab:blue}{HM{[}$\mathcal{R},\mathcal{M}${]}} & 8 & 27.0 & 36.0 & 13.2 & 42.5 & 19.4 & 48.0 & 22.2 & 32.0 & 0.535 & 0.867 & 11.6 & 10.4 & 19.3 & 2.9 & 35.1\tabularnewline
\rowcolor{black!7}\cellcolor{white} \multirow{-2}{*}{CUB} & HM{[}$\mathcal{R},\mathcal{M}${]}\&ICS & 8 & 25.6 & 34.3 & 12.5 & 41.8 & 21.9 & 41.0 & 23.6 & 26.4 & 0.497 & 0.766 & 14.5 & 13.0 & 21.8 & 4.7 & 39.0\tabularnewline
\hline 
& \textcolor{tab:red}{HM{[}$\mathcal{S},\mathcal{M}${]}} & 8 & 38.4 & 49.7 & 22.9 & 50.3 & 10.9 & 50.5 & 10.8 & 44.6 & 0.680 & 0.722 & 13.3 & 11.2 & 25.8 & 1.2 & 29.6\tabularnewline
\rowcolor{black!7}\cellcolor{white}\multirow{-2}{*}{CUB}  & HM{[}$\mathcal{S},\mathcal{M}${]}\&ICS & 8 & 36.9 & 48.9 & 21.6 & 48.8 & 12.4 & 42.9 & 12.5 & 36.6 & 0.850 & 0.446 & 17.0 & 13.9 & 27.2 & 1.9 & 32.3\tabularnewline
\hline 
& HM{[}$\mathcal{R},g_{\mathsf{LGA}}${]} & 8 & 24.8 & 33.9 & 12.2 & 41.6 & 21.4 & 45.0 & 21.7 & 31.3 & 0.452 & 0.846 & 13.2 & 12.0 & 20.9 & 4.6 & 37.3\tabularnewline
\rowcolor{black!7}\cellcolor{white}\multirow{-2}{*}{CUB}  & HM{[}$\mathcal{R},g_{\mathsf{LGA}}${]}\&ICS & 8 & 25.7 & 35.2 & 12.8 & 41.7 & 22.1 & 37.1 & 23.4 & 23.7 & 0.464 & 0.725 & 14.5 & 13.3 & 21.1 & 5.3 & 40.2\tabularnewline
\hline 
& \textcolor{tab:pink}{HM{[}$\mathcal{S},g_{\mathsf{LGA}}${]}} & 8 & 38.0 & 48.3 & 21.8 & 49.3 & 12.7 & 46.4 & 11.6 & 39.9 & 0.567 & 0.783 & 16.8 & 11.9 & 27.9 & 1.4 & 32.4\tabularnewline
\rowcolor{black!7}\cellcolor{white} & \textcolor{crimson}{HM{[}$\mathcal{S},g_{\mathsf{LGA}}${]}\&ICS} & 8 & 37.2 & 47.8 & 21.4 & 48.4 & 12.9 & 40.9 & 14.7 & 33.7 & 0.806 & 0.487 & 17.1 & 13.2 & 26.3 & 2.3 & 33.5\tabularnewline
\multirow{-3}{*}{CUB} & HM{[}$\mathcal{S},g_{\mathsf{LGA}}${]}\&ICS($\lambda{=}1.0$) & 8 & 36.0 & 46.7 & 20.7 & 48.0 & 14.2 & 41.0 & 15.1 & 31.7 & 0.907 & 0.329 & 17.0 & 14.2 & 24.5 & 2.1 & 33.7\tabularnewline
\hline 
\rowcolor{black!7}\cellcolor{white}& \textcolor{crimson}{HM{[}$\mathcal{S},g_{\mathsf{LGA}}${]}\&ICS} & 2 & 45.2 & 57.2 & 28.5 & 53.7 & 3.0 & 79.9 & 2.4 & 78.9 & 0.936 & 0.609 & 3.6 & 1.2 & 19.9 & 0.0 & 15.2\tabularnewline
 & \textcolor{crimson}{HM{[}$\mathcal{S},g_{\mathsf{LGA}}${]}\&ICS} & 4 & 41.8 & 53.0 & 25.3 & 52.0 & 8.1 & 57.3 & 7.9 & 54.1 & 0.892 & 0.514 & 9.8 & 6.7 & 22.9 & 0.5 & 24.6\tabularnewline
\rowcolor{black!7}\cellcolor{white} & \textcolor{crimson}{HM{[}$\mathcal{S},g_{\mathsf{LGA}}${]}\&ICS} & 8 & 37.2 & 47.8 & 21.4 & 48.4 & 12.9 & 40.9 & 14.7 & 33.7 & 0.806 & 0.487 & 17.1 & 13.2 & 26.3 & 2.3 & 33.5\tabularnewline
 & \textcolor{crimson}{HM{[}$\mathcal{S},g_{\mathsf{LGA}}${]}\&ICS} & 16 & 35.5 & 46.4 & 20.4 & 47.5 & 14.9 & 37.2 & 17.1 & 30.3 & 0.771 & 0.495 & 18.2 & 15.3 & 28.7 & 2.8 & 36.0\tabularnewline
\rowcolor{black!7}\cellcolor{white}\multirow{-5}{*}{CUB}  & \textcolor{crimson}{HM{[}$\mathcal{S},g_{\mathsf{LGA}}${]}\&ICS} & 32 & 34.9 & 45.0 & 19.8 & 47.1 & 15.5 & 37.7 & 16.6 & 30.9 & 0.753 & 0.506 & 17.9 & 16.7 & 27.3 & 2.9 & 36.0\tabularnewline

	\bottomrule

\end{tabular}

	}
	\vspace{-0.8em}
\caption{Intra-class structure loss in conjunction with hardness manipulation for adversarial training of a DML Model.}
\label{tab:ics}
\end{table*}



==> cvpr2023-author_kit-v1_1-1/all/tab-sota.tex <==
\begin{table*}
\resizebox{\linewidth}{!}{
\setlength{\tabcolsep}{0.47em}
\renewcommand{\arraystretch}{1.05}%

\begin{tabular}{c|cc|cccc|ccccc|ccccc|c}

	\toprule

\rowcolor{black!12} & & & \multicolumn{4}{c|}{\textbf{Benign Example}} & \multicolumn{10}{c|}{\textbf{White-Box Attacks for Robustness Evaluation}} & \tabularnewline
\cline{4-17} \cline{5-17} \cline{6-17} \cline{7-17} \cline{8-17} \cline{9-17} \cline{10-17} \cline{11-17} \cline{12-17} \cline{13-17} \cline{14-17} \cline{15-17} \cline{16-17} \cline{17-17}
\rowcolor{black!12}\multirow{-2}{*}{\textbf{Dataset}} & \multirow{-2}{*}{\textbf{Defense}} & \multirow{-2}{*}{$\eta$} & R@1$\uparrow$ & R@2$\uparrow$ & mAP$\uparrow$ & NMI$\uparrow$ & CA+$\uparrow$ & CA-$\downarrow$ & QA+$\uparrow$ & QA-$\downarrow$ & TMA$\downarrow$ & ES:D$\downarrow$ & ES:R$\uparrow$ & LTM$\uparrow$ & GTM$\uparrow$ & GTT$\uparrow$ & \multirow{-2}{*}{\textbf{ERS$\uparrow$}}\tabularnewline

	\midrule

& N/A{[}$\mathcal{R}${]} & N/A & 53.9 & 66.4 & 26.1 & 59.5 & 0.0 & 100.0 & 0.0 & 99.9 & 0.883 & 1.762 & 0.0 & 0.0 & 14.1 & 0.0 & 3.8\tabularnewline
\cline{2-18} \cline{3-18} \cline{4-18} \cline{5-18} \cline{6-18} \cline{7-18} \cline{8-18} \cline{9-18} \cline{10-18} \cline{11-18} \cline{12-18} \cline{13-18} \cline{14-18} \cline{15-18} \cline{16-18} \cline{17-18} \cline{18-18} 
 & EST{[}$\mathcal{R}${]}~\cite{advrank} & 8 & 37.1 & 47.3 & 20.0 & 46.4 & 0.5 & 97.3 & 0.5 & 91.3 & 0.875 & 1.325 & 3.9 & 0.4 & 14.9 & 0.0 & 7.9\tabularnewline
\rowcolor{black!7}\cellcolor{white} & \textcolor{cyan}{ACT{[}$\mathcal{R}${]}}~\cite{robrank} & 8 & 30.6 & 40.1 & 16.5 & 45.6 & 13.7 & 46.8 & 12.6 & 39.3 & 0.547 & 0.902 & 13.6 & 9.8 & 21.9 & 1.3 & 31.3\tabularnewline
& \textcolor{tab:pink}{HM{[}$\mathcal{S},g_{\mathsf{LGA}}${]}} & 8 & 38.0 & 48.3 & 21.8 & 49.3 & 12.7 & 46.4 & 11.6 & 39.9 & 0.567 & 0.783 & 16.8 & 11.9 & 27.9 & 1.4 & 32.4\tabularnewline
\rowcolor{black!7}\cellcolor{white} & \textcolor{crimson}{HM{[}$\mathcal{S},g_{\mathsf{LGA}}${]}\&ICS} & 8 & 37.2 & 47.8 & 21.4 & 48.4 & 12.9 & 40.9 & 14.7 & 33.7 & 0.806 & 0.487 & 17.1 & 13.2 & 26.3 & 2.3 & 33.5\tabularnewline
\cline{2-18} \cline{3-18} \cline{4-18} \cline{5-18} \cline{6-18} \cline{7-18} \cline{8-18} \cline{9-18} \cline{10-18} \cline{11-18} \cline{12-18} \cline{13-18} \cline{14-18} \cline{15-18} \cline{16-18} \cline{17-18} \cline{18-18} 
 & EST{[}$\mathcal{R}${]}~\cite{advrank} & 32 & 8.5 & 13.0 & 2.6 & 25.2 & 2.7 & 97.9 & 0.4 & 97.3 & 0.848 & 1.576 & 1.4 & 0.0 & 4.0 & 0.0 & 5.3\tabularnewline
\rowcolor{black!7}\cellcolor{white} & \textcolor{cyan}{ACT{[}$\mathcal{R}${]}}~\cite{robrank} & 32 & 27.5 & 38.2 & 12.2 & 43.0 & 15.5 & 37.7 & 15.1 & 32.2 & 0.472 & 0.821 & 11.1 & 9.4 & 14.9 & 1.0 & 33.9\tabularnewline
& \textcolor{tab:pink}{HM{[}$\mathcal{S},g_{\mathsf{LGA}}${]}} & 32 & 36.5 & 46.7 & 21.0 & 48.6 & 14.7 & 39.6 & 15.6 & 34.2 & 0.523 & 0.736 & 16.5 & 15.0 & 26.7 & 2.9 & 35.9\tabularnewline
\rowcolor{black!7}\cellcolor{white}\multirow{-9}{*}{CUB} & \textcolor{crimson}{HM{[}$\mathcal{S},g_{\mathsf{LGA}}${]}\&ICS} & 32 & 34.9 & 45.0 & 19.8 & 47.1 & 15.5 & 37.7 & 16.6 & 30.9 & 0.753 & 0.506 & 17.9 & 16.7 & 27.3 & 2.9 & 36.0\tabularnewline

	\midrule 

& N/A{[}$\mathcal{R}${]} & N/A & 62.5 & 74.0 & 23.8 & 57.0 & 0.2 & 100.0 & 0.1 & 99.6 & 0.874 & 1.816 & 0.0 & 0.0 & 13.4 & 0.0 & 3.6\tabularnewline
\cline{2-18} \cline{3-18} \cline{4-18} \cline{5-18} \cline{6-18} \cline{7-18} \cline{8-18} \cline{9-18} \cline{10-18} \cline{11-18} \cline{12-18} \cline{13-18} \cline{14-18} \cline{15-18} \cline{16-18} \cline{17-18} \cline{18-18} 
 & EST{[}$\mathcal{R}${]}~\cite{advrank} & 8 & 57.1 & 68.4 & 30.3 & 47.7 & 0.1 & 99.9 & 0.1 & 98.1 & 0.902 & 1.681 & 0.7 & 0.2 & 15.4 & 0.0 & 4.4\tabularnewline
\rowcolor{black!7}\cellcolor{white} & \textcolor{cyan}{ACT{[}$\mathcal{R}${]}}~\cite{robrank} & 8 & 46.8 & 58.0 & 23.4 & 45.5 & 19.3 & 33.1 & 20.3 & 32.3 & 0.413 & 0.760 & 18.4 & 15.0 & 28.6 & 1.2 & 39.8\tabularnewline
& \textcolor{tab:pink}{HM{[}$\mathcal{S},g_{\mathsf{LGA}}${]}} & 8 & 63.2 & 73.7 & 36.8 & 53.5 & 15.3 & 32.0 & 17.9 & 33.9 & 0.463 & 0.653 & 23.4 & 28.5 & 44.6 & 5.8 & 42.4\tabularnewline
\rowcolor{black!7}\cellcolor{white} & \textcolor{crimson}{HM{[}$\mathcal{S},g_{\mathsf{LGA}}${]}\&ICS} & 8 & 61.7 & 72.6 & 35.5 & 51.8 & 21.0 & 23.3 & 23.1 & 22.2 & 0.698 & 0.415 & 31.2 & 38.0 & 47.8 & 9.6 & 47.9\tabularnewline
\cline{2-18} \cline{3-18} \cline{4-18} \cline{5-18} \cline{6-18} \cline{7-18} \cline{8-18} \cline{9-18} \cline{10-18} \cline{11-18} \cline{12-18} \cline{13-18} \cline{14-18} \cline{15-18} \cline{16-18} \cline{17-18} \cline{18-18} 
 & EST{[}$\mathcal{R}${]}~\cite{advrank} & 32 & 30.7 & 41.0 & 5.6 & 31.8 & 1.2 & 98.1 & 0.4 & 91.8 & 0.880 & 1.281 & 2.9 & 0.7 & 8.2 & 0.0 & 7.3\tabularnewline
\rowcolor{black!7}\cellcolor{white} & \textcolor{cyan}{ACT{[}$\mathcal{R}${]}}~\cite{robrank} & 32 & 43.4 & 54.6 & 11.8 & 42.9 & 18.0 & 32.3 & 17.5 & 30.5 & 0.383 & 0.763 & 16.3 & 15.3 & 20.7 & 1.6 & 38.6\tabularnewline
& \textcolor{tab:pink}{HM{[}$\mathcal{S},g_{\mathsf{LGA}}${]}} & 32 & 62.3 & 72.5 & 35.3 & 52.7 & 17.4 & 28.2 & 18.2 & 28.8 & 0.426 & 0.613 & 27.1 & 30.7 & 42.3 & 7.9 & 44.9\tabularnewline
\rowcolor{black!7}\cellcolor{white}\multirow{-9}{*}{CARS} & \textcolor{crimson}{HM{[}$\mathcal{S},g_{\mathsf{LGA}}${]}\&ICS} & 32 & 60.2 & 71.6 & 33.9 & 51.2 & 19.3 & 25.9 & 19.6 & 25.7 & 0.650 & 0.446 & 30.3 & 36.7 & 46.0 & 8.8 & 46.0\tabularnewline

	\midrule

& N/A{[}$\mathcal{R}${]} & N/A & 62.9 & 68.5 & 39.2 & 87.4 & 0.1 & 99.3 & 0.2 & 99.1 & 0.845 & 1.685 & 0.0 & 0.0 & 6.3 & 0.0 & 4.0\tabularnewline
\cline{2-18} \cline{3-18} \cline{4-18} \cline{5-18} \cline{6-18} \cline{7-18} \cline{8-18} \cline{9-18} \cline{10-18} \cline{11-18} \cline{12-18} \cline{13-18} \cline{14-18} \cline{15-18} \cline{16-18} \cline{17-18} \cline{18-18} 
 & EST{[}$\mathcal{R}${]}~\cite{advrank} & 8 & 52.7 & 58.5 & 30.1 & 85.7 & 6.4 & 69.7 & 3.9 & 64.6 & 0.611 & 1.053 & 3.8 & 2.2 & 10.2 & 1.3 & 19.0\tabularnewline
\rowcolor{black!7}\cellcolor{white} & \textcolor{cyan}{ACT{[}$\mathcal{R}${]}}~\cite{robrank} & 8 & 45.3 & 50.6 & 24.1 & 84.7 & 24.8 & 10.7 & 25.4 & 8.2 & 0.321 & 0.485 & 15.4 & 17.7 & 25.1 & 11.3 & 49.5\tabularnewline
& \textcolor{tab:pink}{HM{[}$\mathcal{S},g_{\mathsf{LGA}}${]}} & 8 & 49.0 & 54.1 & 26.4 & 85.0 & 29.9 & 4.7 & 31.6 & 3.6 & 0.455 & 0.283 & 39.3 & 40.9 & 38.8 & 43.0 & 61.7\tabularnewline
\rowcolor{black!7}\cellcolor{white} & \textcolor{crimson}{HM{[}$\mathcal{S},g_{\mathsf{LGA}}${]}\&ICS} & 8 & 48.3 & 53.4 & 25.7 & 84.9 & 32.5 & 4.8 & 32.4 & 3.5 & 0.586 & 0.239 & 38.6 & 39.8 & 38.3 & 44.5 & 61.2\tabularnewline
\cline{2-18} \cline{3-18} \cline{4-18} \cline{5-18} \cline{6-18} \cline{7-18} \cline{8-18} \cline{9-18} \cline{10-18} \cline{11-18} \cline{12-18} \cline{13-18} \cline{14-18} \cline{15-18} \cline{16-18} \cline{17-18} \cline{18-18} 
 & EST{[}$\mathcal{R}${]}~\cite{advrank} & 32 & 46.0 & 51.4 & 24.5 & 84.7 & 12.5 & 43.6 & 10.6 & 34.8 & 0.468 & 0.830 & 9.6 & 7.2 & 17.3 & 3.8 & 31.7\tabularnewline
\rowcolor{black!7}\cellcolor{white} & \textcolor{cyan}{ACT{[}$\mathcal{R}${]}}~\cite{robrank} & 32 & 47.5 & 52.6 & 25.5 & 84.9 & 24.1 & 10.5 & 22.7 & 9.4 & 0.253 & 0.532 & 21.2 & 21.6 & 27.8 & 15.3 & 50.8\tabularnewline
& \textcolor{tab:pink}{HM{[}$\mathcal{S},g_{\mathsf{LGA}}${]}} & 32 & 47.7 & 52.7 & 25.3 & 84.8 & 30.6 & 4.7 & 31.2 & 3.5 & 0.466 & 0.266 & 38.6 & 40.3 & 38.6 & 44.3 & 61.8\tabularnewline
\rowcolor{black!7}\cellcolor{white}\multirow{-9}{*}{SOP} & \textcolor{crimson}{HM{[}$\mathcal{S},g_{\mathsf{LGA}}${]}\&ICS} & 32 & 46.8 & 51.7 & 24.5 & 84.7 & 32.0 & 4.2 & 33.7 & 3.0 & 0.606 & 0.207 & 39.1 & 39.8 & 37.9 & 45.6 & 61.6\tabularnewline

	\bottomrule

\end{tabular}}
	\vspace{-0.8em}
\caption{Comparison of our defense with the state-of-the-art methods on commonly used DML datasets.}
	\label{tab:sota}
	\vspace{-0.4em}
\end{table*}


==> cvpr2023-author_kit-v1_1-1/all/tab-srcdest.tex <==
\begin{table*}
\resizebox{\linewidth}{!}{
\setlength{\tabcolsep}{0.48em}%
\begin{tabular}{c|cc|cccc|ccccc|ccccc|c}

	\toprule

\multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Defense}} & \multirow{2}{*}{$\eta$} & \multicolumn{4}{c|}{\textbf{Benign Example}} & \multicolumn{10}{c|}{\textbf{White-Box Attacks for Robustness Evaluation}} & \multirow{2}{*}{\textbf{ERS}}\tabularnewline
\cline{4-17} \cline{5-17} \cline{6-17} \cline{7-17} \cline{8-17} \cline{9-17} \cline{10-17} \cline{11-17} \cline{12-17} \cline{13-17} \cline{14-17} \cline{15-17} \cline{16-17} \cline{17-17} 
 &  &  & R@1$\uparrow$ & R@2$\uparrow$ & mAP$\uparrow$ & NMI$\uparrow$ & CA+$\uparrow$ & CA-$\downarrow$ & QA+$\uparrow$ & QA-$\downarrow$ & TMA$\downarrow$ & ES:D$\downarrow$ & ES:R$\uparrow$ & LTM$\uparrow$ & GTM$\uparrow$ & GTT$\uparrow$ & \tabularnewline

	\midrule

\multirow{5}{*}{CUB} & HM{[}$\mathcal{R},\mathcal{R}${]} & N/A & 53.9 & 66.4 & 26.1 & 59.5 & 0.0 & 100.0 & 0.0 & 99.9 & 0.883 & 1.762 & 0.0 & 0.0 & 14.1 & 0.0 & 3.8\tabularnewline
 & HM{[}$\mathcal{R},\mathcal{M}${]} & 8 & 27.0 & 36.0 & 13.2 & 42.5 & 19.4 & 48.0 & 22.2 & 32.0 & 0.535 & 0.867 & 11.6 & 10.4 & 19.3 & 2.9 & 35.1\tabularnewline
 & HM{[}$\mathcal{R},\mathcal{S}${]} & 8 & C & o & l & l & a & p & s & e &  &  &  &  &  &  & \tabularnewline
 & HM{[}$\mathcal{R},\mathcal{D}${]} & 8 & C & o & l & l & a & p & s & e &  &  &  &  &  &  & \tabularnewline
 & HM{[}$\mathcal{R},\mathcal{H}${]} & 8 & C & o & l & l & a & p & s & e &  &  &  &  &  &  & \tabularnewline
\hline 
\multirow{5}{*}{CUB} & HM{[}$\mathcal{M},\mathcal{R}${]} & 8 & 43.9 & 55.9 & 27.1 & 54.2 & 0.2 & 100.0 & 0.4 & 99.6 & 0.849 & 1.640 & 0.2 & 0.1 & 19.1 & 0.0 & 5.4\tabularnewline
 & HM{[}$\mathcal{M},\mathcal{M}${]} & N/A & 44.0 & 56.1 & 27.2 & 54.6 & 0.1 & 100.0 & 0.4 & 99.8 & 0.843 & 1.717 & 0.3 & 0.3 & 18.4 & 0.0 & 5.0\tabularnewline
 & HM{[}$\mathcal{M},\mathcal{S}${]} & 8 & C & o & l & l & a & p & s & e &  &  &  &  &  &  & \tabularnewline
 & HM{[}$\mathcal{M},\mathcal{D}${]} & 8 & C & o & l & l & a & p & s & e &  &  &  &  &  &  & \tabularnewline
 & HM{[}$\mathcal{M},\mathcal{H}${]} & 8 & C & o & l & l & a & p & s & e &  &  &  &  &  &  & \tabularnewline
\hline 
\multirow{5}{*}{CUB} & HM{[}$\mathcal{S},\mathcal{R}${]} & 8 & 48.3 & 60.1 & 30.3 & 56.3 & 2.0 & 84.4 & 1.4 & 85.4 & 0.835 & 0.895 & 6.1 & 1.6 & 21.0 & 0.0 & 13.7\tabularnewline
 & HM{[}$\mathcal{S},\mathcal{M}${]} & 8 & 38.4 & 49.7 & 22.9 & 50.3 & 10.9 & 50.5 & 10.8 & 44.6 & 0.680 & 0.722 & 13.3 & 11.2 & 25.8 & 1.2 & 29.6\tabularnewline
 & HM{[}$\mathcal{S},\mathcal{S}${]} & N/A & 55.7 & 68.2 & 35.8 & 61.0 & 0.0 & 100.0 & 0.0 & 99.6 & 0.942 & 1.272 & 0.0 & 0.0 & 19.2 & 0.0 & 6.2\tabularnewline
 & HM{[}$\mathcal{S},\mathcal{D}${]} & 8 & C & o & l & l & a & p & s & e &  &  &  &  &  &  & \tabularnewline
 & HM{[}$\mathcal{S},\mathcal{H}${]} & 8 & C & o & l & l & a & p & s & e &  &  &  &  &  &  & \tabularnewline
\hline 
\multirow{5}{*}{CUB} & HM{[}$\mathcal{D},\mathcal{R}${]} & 8 & 52.7 & 64.0 & 33.7 & 58.9 & 0.0 & 100.0 & 0.2 & 100.0 & 0.841 & 1.749 & 0.1 & 0.0 & 19.0 & 0.0 & 4.8\tabularnewline
 & HM{[}$\mathcal{D},\mathcal{M}${]} & 8 & 50.7 & 63.8 & 33.1 & 58.7 & 0.0 & 100.0 & 0.3 & 99.9 & 0.841 & 1.744 & 0.2 & 0.0 & 18.5 & 0.0 & 4.8\tabularnewline
 & HM{[}$\mathcal{D},\mathcal{S}${]} & 8 & C & o & l & l & a & p & s & e &  &  &  &  &  &  & \tabularnewline
 & HM{[}$\mathcal{D},\mathcal{D}${]} & N/A & 51.4 & 64.2 & 33.4 & 59.3 & 0.0 & 100.0 & 0.4 & 99.9 & 0.842 & 1.753 & 0.0 & 0.0 & 19.7 & 0.0 & 4.9\tabularnewline
 & HM{[}$\mathcal{D},\mathcal{H}${]} & 8 & 54.7 & 66.9 & 36.2 & 60.0 & 0.0 & 100.0 & 0.2 & 99.8 & 0.874 & 1.569 & 0.4 & 0.0 & 18.6 & 0.0 & 5.4\tabularnewline
\hline 
\multirow{5}{*}{CUB} & HM{[}$\mathcal{H},\mathcal{R}${]} & 8 & 51.0 & 63.5 & 32.9 & 59.2 & 0.0 & 100.0 & 0.2 & 99.9 & 0.837 & 1.750 & 0.0 & 0.0 & 17.7 & 0.0 & 4.7\tabularnewline
 & HM{[}$\mathcal{H},\mathcal{M}${]} & 8 & 52.2 & 64.0 & 33.1 & 58.4 & 0.0 & 100.0 & 0.2 & 100.0 & 0.841 & 1.750 & 0.0 & 0.0 & 18.9 & 0.0 & 4.8\tabularnewline
 & HM{[}$\mathcal{H},\mathcal{S}${]} & 8 & C & o & l & l & a & p & s & e &  &  &  &  &  &  & \tabularnewline
 & HM{[}$\mathcal{H},\mathcal{D}${]} & 8 & 52.6 & 64.9 & 34.4 & 60.0 & 0.0 & 100.0 & 0.2 & 99.9 & 0.835 & 1.720 & 0.1 & 0.0 & 20.0 & 0.0 & 5.1\tabularnewline
 & HM{[}$\mathcal{H},\mathcal{H}${]} & N/A & 48.9 & 61.2 & 30.3 & 56.5 & 0.0 & 100.0 & 0.4 & 99.9 & 0.830 & 1.752 & 0.2 & 0.0 & 19.5 & 0.0 & 5.0\tabularnewline

	\bottomrule

\end{tabular}}

	\caption{Full data sheet for Tab.2 in the Paper. The symbols $\mathcal{R},
	\mathcal{M}, \mathcal{S}, \mathcal{D}, \mathcal{H}$ denote Random, Semihard,
	Softhard, Distance and Hardest triplet sampling strategies, respectively.
	%
	Experiments that end up with model collapse are left with a placeholder 
	in the table.
	}
\label{tab:srcdest}
\end{table*}

